Behaviour Driven Development: A Systematic Mapping Study

Context: Behaviour Driven Development (BDD) uses scenarios written in semi-structured natural language to express software requirements in a way that can be understood by all stakeholders. The resulting natural language specifications can also be executed to reveal correct and problematic parts of a software. Although BDD was introduced about two decades ago, there is a lack of secondary studies in peer-reviewed scientific literature. Objective: To understand the current state of BDD research by conducting a systematic mapping study that covers studies published from 2006 to 2021. Method: By following the guidelines for conducting systematic mapping studies in software engineering, we sought to answer research questions on types of venues in which BDD papers have been published, research, contributions, studied topics and their evolution, and evaluation methods used in published BDD research. Results: The study identified 166 papers which were mapped. Key results include the following: the dominance of conference papers; scarcity of research with insights from the industry; shortage of philosophical papers on BDD; acute shortage of metrics for measuring various aspects of BDD specifications and the processes for producing BDD specifications; the dominance of studies on using BDD for facilitating various software development endeavours, improving the BDD process and associated artefacts, and applying BDD in different contexts; scarcity of studies on using BDD alongside other software techniques and technologies; increase in diversity of studied BDD topics; and notable use of case studies and experiments to study different BDD aspects. Conclusion: The paper improves our understanding of the state of the art of BDD, and highlights important areas of focus for future BDD research.

==> themes.tex <==
\section{Themes}
The following are the themes identified as well as their sub-themes: 
\begin{enumerate}
\item BDD and other processes
    \begin{enumerate}
    \item  BDD comparison
    \item BDD and scrum
    \item DevOps
    \end{enumerate}
\item Context/application area
\begin{enumerate}
    \item Multi-agent systems
    \item Hardware context
    \item Health context
    \item Education context
    \item BDD and Networking
    \item Product configuration systems
    \item Mobile apps
    \item Enterprise systems
\end{enumerate}
\item{Technologies}
\begin{enumerate}
    \item Micro services
    \item Block chain
    \item Web services
    \item Machine learning
\end{enumerate}
\item{Techniques}
\begin{enumerate}
    \item Ontology
\end{enumerate}
\item BDD to facilitate
    \begin{enumerate}
        \item Safety
        \item GUI Testing
        \item Spread sheets testing — application area?
        \item Product lines
         \item Compliance testing
        \item Traceability
        \item Model Testing
        \item Business process modelling
        \item Test selection
        \item Usability testing
        \item Security and privacy
        \item Model-based testing
        \item Artifact generation  — could also be in studies on improving the BDD process
        \item Integration testing
        \item Load testing
        \item Syntax highlighting
        \item Reproducing bugs
    \end{enumerate}
\item Studies on improving the BDD process itself
\begin{enumerate}
    \item  Specification quality
    \item  Specification language
    \item  Refactoring
    \item  Duplicate detection
    \item  Co evolution of BDD artifacts
    \item  BDD Adoption
    \item  BDD characteristics
    \item  Test cases used as requirements — check if we can merge this with another theme
    \item  Use of BDD tools — Merge with adoption?
\end{enumerate}
\end{enumerate}

